Evaluating the Utility of Anonymized Network Traces for Intrusion Detection

Anonymization is the process of removing or hiding sensitive information in logs. Anonymization allows organizations to share network logs while not exposing sensitive information. However, there is an inherent trade off between the amount of information revealed in the log and the usefulness of the log to the client (the utility of a log). There are many anonymization techniques, and there are many ways to anonymize a particular log (that is, which fields to anonymize and how). Different anonymization policies will result in logs with varying levels of utility for analysis. In this paper we explore the effect of different anonymization policies on logs. We provide an empirical analysis of the effect of varying anonymization policies by looking at the number of alerts generated by an Intrusion Detection System. This is the first work to thoroughly evaluate the effect of single field anonymization policies on a data set. Our main contributions are to determine a set of fields that have a large impact on the utility of a log.

==> MarginalAnonyAlerts-FP-FN-Error.tex <==
\begin{table*}
  \begin{tabular}[t]{lcccccc} \textbf{AnonyAlg}& \textbf{AvgAlerts} &
    \textbf{MaxAlerts}& \textbf{MinAlerts}& \textbf{AvgFP} &
    \textbf{AvgFN} & \textbf{AvgError} \\
    Substitution&461341.5&923033&81&461298.5&38&5695.51 \\
    Classify&50273.33&521670&81&50205.33&13&619.98 \\
    Annihilation&47383.08&923033&5&47316.41&14.33&584.33 \\
    NumericTruncation&32755.17&457410&5&32698.43&24.26&403.98 \\
    BinaryBlackMarker&30094.93&520290&5&30032.7&18.77&371.01 \\
    IPv4PrefixPreserving&403.2&1014&81&351&28.8&4.69 \\
    TimeEnumeration&160.5&399&81&80.75&1.25&1.01 \\
    TimeUnitAnnihilation&81&81&81&0&0&0 \\
    BytesTruncation&81&81&81&0&0&0 \\
    RandomTimeShift&81&81&81&0&0&0 \\
    MacRandomPermutation&81&81&81&0&0&0 \\
    RandomPermutation&66.39&81&9&6.61&21.22&0.34 \\
  \end{tabular}
  \caption{Average number of alerts generated over all anonymization
    algorithms applied to a field. \textbf{AnonyAlg} is the anonymization algorithm being
    anonymized, \textbf{AvgAlerts} is the average number of alerts
    generated, \textbf{MaxAlerts} is the maximum number of alerts
    generated. \textbf{MinAlerts} is the minimum number of alerts
    generated.  \textbf{AvgFP} is the average number of false positives. \textbf{AvgFN} is the average number of false negatives. \textbf{AvgError} is the average error. }
  \label{table:marginal-anony-alerts}
\end{table*}

==> MarginalFieldAlerts-AlertsStd.tex <==
\begin{table*}
\begin{tabular}[t]{lcccc}
  \textbf{Field}&\textbf{AvgAlerts}&\textbf{MaxAlerts}&\textbf{MinAlerts}&\textbf{StDAlerts} \\ 
  IPV4\_ID&81&81&81&0 \\ 
  UDP\_CHECKSUM&81&81&81&0 \\ 
  IPV4\_OFFSET&81&81&81&0 \\ 
  IPV4\_TTL&81&81&81&0 \\ 
  SRC\_MAC&81&81&81&0 \\ 
  DST\_MAC&81&81&81&0 \\ 
  UDP\_DST\_PORT&81&81&81&0 \\ 
  TCP\_DST\_PORT&557575.67&923033&18&343715.37 \\ 
  TCP\_WINDOW&81&81&81&0 \\ 
  TCP\_SRC\_PORT&483560.33&922171&20&367490.47 \\ 
  TS\_USEC&81&81&81&0 \\ 
  TCP\_CHECKSUM&81&81&81&0 \\ 
  TCP\_URGENT&81&81&81&0 \\ 
  TS\_SEC&145&399&81&141.99 \\ 
  IPV4\_CHECKSUM&81&81&81&0 \\ 
  IPV4\_DST\_IP&160&759&9&334.86 \\ 
  TCP\_ACK\_NO&63.75&81&56&11.84 \\ 
  TCP\_FLAGS&5&5&5&0 \\ 
  UDP\_SRC\_PORT&81&81&81&0 \\ 
  TCP\_SEQUENCE&73&81&65&9.24 \\ 
  TCP\_OPTIONS&81&81&81&0 \\ 
  IPV4\_SRC\_IP&210&1014&9&449.45 \\ 
\end{tabular}
\caption{Average number of alerts generated over all anonymization
  algorithms applied to a field. This table includes the standard deviation in alerts generated over all the anonymization algorithms. \textbf{Field} is the field being
  anonymized, \textbf{AvgAlerts} is the average number of alerts
  generated, \textbf{MaxAlerts} is the maximum number of alerts
  generated. \textbf{MinAlerts} is the minimum number of alerts
  generated. \textbf{StdAlerts} is the standard deviation in the number of alerts generated }
  \label{table:marginal-field-alerts-std}
\end{table*}

==> MarginalFieldAlerts-FP-FN-Error.tex <==
\begin{table*}
\begin{tabular}[t]{lcccccc}
\textbf{Field}&\textbf{AvgAlerts}&\textbf{MaxAlerts}&\textbf{MinAlerts}&\textbf{AvgFP} & \textbf{AvgFN} & \textbf{AvgError} \\ 
TCP\_DST\_PORT&557575.67&923033&18&557572.33&77.67&6884.57 \\ 
TCP\_SRC\_PORT&483560.33&922171&20&483554.83&75.5&5970.74 \\ 
IPV4\_SRC\_IP&210&1014&9&201&72&3.37 \\ 
IPV4\_DST\_IP&160&759&9&151&72&2.75 \\ 
IPV4\_ID&81&81&81&80.6&80.6&1.99 \\ 
TCP\_SEQUENCE&73&81&65&52&60&1.38 \\ 
TCP\_FLAGS&5&5&5&0&76&0.94 \\ 
TS\_SEC&145&399&81&65.2&1.2&0.82 \\ 
TCP\_ACK\_NO&63.75&81&56&3&20.25&0.29 \\ 
\emph{DST\_MAC}&81&81&81&0&0&0 \\ 
\emph{IPV4\_CHECKSUM}&81&81&81&0&0&0 \\ 
\emph{IPV4\_OFFSET}&81&81&81&0&0&0 \\ 
\emph{IPV4\_TTL}&81&81&81&0&0&0 \\ 
\emph{SRC\_MAC}&81&81&81&0&0&0 \\ 
\emph{TCP\_CHECKSUM}&81&81&81&0&0&0 \\ 
\emph{TCP\_OPTIONS}&81&81&81&0&0&0 \\ 
\emph{TCP\_URGENT}&81&81&81&0&0&0 \\ 
\emph{TCP\_WINDOW}&81&81&81&0&0&0 \\ 
\emph{TS\_USEC}&81&81&81&0&0&0 \\ 
\emph{UDP\_CHECKSUM}&81&81&81&0&0&0 \\ 
\emph{UDP\_DST\_PORT}&81&81&81&0&0&0 \\ 
\emph{UDP\_SRC\_PORT}&81&81&81&0&0&0 \\ 
\end{tabular}
\caption{Average number of alerts generated over all anonymization algorithms applied to a field. \textbf{Field} is the field being anonymized, \textbf{AvgAlerts} is the average number of alerts generated, \textbf{MaxAlerts} is the maximum number of alerts generated. \textbf{MinAlerts} is the minimum number of alerts generated. \textbf{AvgFP} is the average number of false positives. \textbf{AvgFN} is the average number of false negatives. \textbf{AvgError} is the average error. The number of alerts generated in the baseline file was 81. }
\label{table:marginal-field-alerts}
\end{table*}


==> MarginalFieldAlerts.tex <==
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "asiaCCS08Anonymization-submit"
%%% End: 
\begin{table*}
\begin{tabular}[t]{lcccc}
\textbf{Field}&\textbf{AvgAlerts}&\textbf{MaxAlerts}&\textbf{MinAlerts}&\textbf{AvgFP} \\ 
TCP\_DST\_PORT&557575.67&923033&18&557572.33 \\ 
TCP\_SRC\_PORT&483560.33&922171&20&483554.83 \\ 
TS\_SEC&145&399&81&65.2 \\ 
IPV4\_SRC\_IP&210&1014&9&201 \\ 
IPV4\_DST\_IP&160&759&9&151 \\ 
TCP\_OPTIONS&81&81&81&0 \\
TCP\_SEQUENCE&73&81&65&52 \\ 
TCP\_ACK\_NO&63.75&81&56&3 \\ 
TCP\_FLAGS&5&5&5&0 \\ 
IPV4\_ID&81&81&81&80.6 \\ 
UDP\_CHECKSUM&81&81&81&0 \\ 
IPV4\_OFFSET&81&81&81&0 \\ 
IPV4\_TTL&81&81&81&0 \\ 
SRC\_MAC&81&81&81&0 \\ 
DST\_MAC&81&81&81&0 \\ 
UDP\_DST\_PORT&81&81&81&0 \\ 
TCP\_WINDOW&81&81&81&0 \\ 
TS\_USEC&81&81&81&0 \\ 
TCP\_CHECKSUM&81&81&81&0 \\ 
TCP\_URGENT&81&81&81&0 \\ 
IPV4\_CHECKSUM&81&81&81&0 \\ 
UDP\_SRC\_PORT&81&81&81&0 \\ 
\end{tabular}
\caption{Average number of alerts generated over all anonymization algorithms applied to a field. \textbf{Field} is the field being anonymized, \textbf{AvgAlerts} is the average number of alerts generated, \textbf{MaxAlerts} is the maximum number of alerts generated. \textbf{MinAlerts} is the minimum number of alerts generated. \textbf{AvgFP} is the average number of false positivesThe number of alerts generated in the baseline file was 81. }
\label{table:marginal-field-alerts}
\end{table*}



==> multifieldData.tex <==
\begin{table*}
  \caption{This table shows that a multi-field policy has uncertain affects on the utility of a log. } 
 \label{tab:multifield}
 \begin{tabular}{ll}
    \textbf{Policy} & \textbf{Alerts} \\
    IPV4\_SRC\_IP-IPv4PrefixPreserving	& 1014 \\
    TCP\_SRC\_PORT-RandomPermutation & 7 \\
    TS\_SEC-TimeEnumeration & 399 \\
    IPV4\_SRC\_IP,TCP\_SRC\_PORT & 1016 \\
    IPV4\_SRC\_IP,TCP\_SRC\_PORT and TS\_SEC & 1010 \\
  \end{tabular} 
\end{table*}

==> rawresultstable.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "asiaCCS08Anonymization-submit"
%%% End: 

\emph{results}

==> results.tex <==
\section{Results and Analysis}
\label{sec:results-analysis}
Our objective was to begin to understand the affect of anonymization on the the utility of a log. There are two factors that affect the utility of a log, the anonymization algorithm and the field which is anonymized. We first look at how the field that is anonymized affects utility. 

We evaluated all 152 pairs of fields and anonymization algorithms. For each pair the number of alerts generated by Snort was calculated. The alerts generated for each pair was compared with the baseline alerts. False Positives/False negatives were calculated based on the definitions above. Table~\ref{table:raw-anony1} and Table~\ref{table:raw-anony2} list the results from most of the pairs of anonymization algorithms and fields.  

ICMP related fields (such as ICMP\_CHECKSUM, ICMP\_COE etc) were excluded since we filtered ICMP packets from the log. There remained a total of 81 field-anonymization pairs.

 
% \begin{minipage}[h]{0.5\linewidth}
%   \begin{titemize}
%   \item ICMP\_CHECKSUM
%     \item ICMP\_COE
%     \item ICMP\_GATEWAY
%     \item ICMP\_IDTENIFIER 
%     \item ICMP\_IPV4\_DST\_IP
%     \item ICMP\_IPV4\_ID 
%     \item ICMP\_IPV4\_SRC\_IP
%   \end{titemize}
% \end{minipage}\begin{minipage}[h]{0.5\linewidth}
%   \begin{titemize}
%     \item  ICMP\_IPV4\_TTL
%     \item ICMP\_ORIG\_DATA
%     \item ICMP\_POINTER    
%     \item ICMP\_SEQUENCE
%     \item ICMP\_ICMP\_TS\_ORIG
%     \item ICMP\_TS\_REC
%     \item ICMP\_TS\_TRANS
%     \item ICMP\_TYPE
%   \end{titemize}
% \end{minipage}

The unanonymized file produced 81 alerts. They number and types of alerts produced are summarized in Table~\ref{table:baseline-alerts}. There are a total of 81 alerts generated in the baseline file, but only 19 unique types of alerts. 

\begin{table}[t]
  \begin{tabular}[t]{llp{2in}}
    {\textbf{AlertID}} & {\textbf{Num}} & \textbf{Desc} \\
    1 & 1 & (portscan) TCP Portscan \footnote{This alert was generated from generator 122} \\
    323 & 1 & FINGER root query \\
    330 & 1 & FINGER redirection attempt \\
    332 & 1 & FINGER 0 query \\
    356 & 1 &  FTP passwd retrieval attempt \\
    359 & 1 & FTP satan scan \\
    503 & 4 & MISC Source Port 20 to <1024 \\
    1200 & 9 & ATTACK-RESPONSES Invalid UR \\
    1201 & 12 & ATTACK-RESPONSES 403 Forbidden \\
    1288 & 4 &  WEB-FRONTPAGE /\_vti\_bin/ access \\
    1292 & 30 &  ATTACK-RESPONSES directory listing \\
    1418 & 2 & SNMP request tcp \\
    1420 & 2 &  SNMP trap tcp \\
    1421 & 1& SNMP AgentX/tcp request\\
    2467 & 1 & NETBIOS SMB D\$ unicode share access \\
    2470 & 1 & NETBIOS SMB C\$ unicode share access \\
    2473 & 1 & NETBIOS SMB ADMIN\$ unicode share access \\
    3151 & 6 &  FINGER / execution attempt \\
    3441 & 2 & FTP PORT bounce attempt \\
  \end{tabular}
  \caption{Alerts generated in the baseline unanonymized file. \textbf{AlertID} is the id of the alert; \textbf{Num} is the number of that type of alert generated; \textbf{Desc} is a description of the alert}
  \label{table:baseline-alerts}
\end{table}



% Two factors influence the utility of a log file, the anonymization algorithm and the field it was applied upon. We start by considering the affect of anonymizing a particular field. 

Table~\ref{table:raw-anony1} and Table~\ref{table:raw-anony2} provided in the Appendix, contain the number of alerts generated for each pair of field and anonymization algorithm. However, we will be focusing on the summarized results here. 

To evaluate the affect of anonymizing a particular field, we combine the alerts generated for a particular field over all the anonymization algorithms applied to it. Table~\ref{table:marginal-field-alerts} shows the number of alerts generated for a field, averaged over all the anonymization algorithms. Table~\ref{table:marginal-field-alerts} also shows the number of false positives, false negatives, and error. 

We can see that several of the fields resulted, in, on average, only 81 alerts. These fields (shown in italics in the table) had 0 error. Judging from these results, we can see that this set of fields did not affect the utility of the log as measured by the IDS metric. 

TCP\_DST\_PORT and TCP\_SRC\_PORT generated the most alerts on average, as well as the most error. Table~\ref{table:raw-anony1} lists the number of alerts for each anonymization algorithm-field pair. We can see that most of the pairs generated only 2 types of alerts. In the case of BinaryBlackMarker there were 520286 alerts of type 524 generated. Alert 524 is ``BAD-TRAFFIC tcp port 0 traffic''. The other anonymization algorithms produced the same pattern --- the majority of alerts were of type 524. 

The reason for this is due to what we substitute for the port field. The BinaryBlackMarker, Substitution, NumericTruncation, and Annihilation algorithms replaced the port field with $0$. This resulted in the alert for nearly all the packets in the log (see Table~\ref{tab:anonyparam} for the parameter settings of the anonymization algorithms). the same problem occurs for the TCP\_SRC\_PORT field. 

The RandomPermutation algorithm replaced the port number with another, random port number, thus not causing the generation of the BAD-TRAFFIC alert. Clearly the choice of parameter setting can cause a large effect on the utility of a log.

Table~\ref{table:marginal-field-alerts} indicates the impact on utility for anonymizing particular fields. From this data, we can determine a rough ordering for fields in terms of their impact on utility. The field that can affect utility most would be the source and destination port fields. However, much of this is due to the parameter settings. Given a ``correct'' parameter setting the alerts might be reduced.

Following the port field are the source and destination ip address fields. It is surprising that the IP address impacts the utility of the log.  The false positive and false negative scores indicate that anonymizing the fields resulted in the generation of alerts outside of the baseline. Table~\ref{table:raw-anony1} indicates some interesting differences between anonymization algorithms. Further investigation is warranted to decide why the IP address causes such an impact.


We can clearly see that the choice of field impacts utility. However, we do not know how the anonymization algorithm affects the utility. We have seen some instances of fields where the choice of anonymization algorithm (and even parameters of the algorithm) can cause large differences. Given this, we would expect significant differences between the utility of two fields anonymized with different algorithms. To detect this difference we calculated the number of alerts generated by a particular anonymization algorithm, over all the fields. The results of this are shown in Table~\ref{table:marginal-anony-alerts}.

However, Table~\ref{table:marginal-anony-alerts} will be skewed by the effect of the field. As can be seen, the five algorithms used to anonymize the port fields have a large number of alerts which overshadow the affect of the algorithms on other fields. 

To get a better look, we looked at the variance of alerts field by field. For each field we calculated the standard deviation of alerts over anonymization algorithms. Table~\ref{table:marginal-field-alerts-std} contains this data. We can see that the choice of anonymization algorithm does affect the utility of a log. The impact of a particular anonymization algorithm needs to be studied further, but it is clear that it does affect the utility. 

\begin{figure*}[t]
  \includegraphics[width=3in]{./img/Field-AvgError.pdf}
  \caption{Graph of error averaged over anonymization algorithm. For every policy take the average error generated over all anonymization algorithms. Note that only the fields TCP\_SRC\_PORT and TCP\_DST\_PORT provide large error. }
\end{figure*}

\begin{figure*}[t]
  \includegraphics[width=3in]{./img/AnonyA-AvgError.pdf}
  \caption{Error averaged over fields. For every policy take the average error generated over all fields. Note that substitution has significantly higer error than the other anonymization algorithms.}
\end{figure*}
\input{rawAlertData.tex}


==> results2-backup.tex <==
\section{Results and Analysis}
\label{sec:results-analysis}

In this section, we describe the results of our experiments with single
field anonymization policies. These experiments provide a substantive
start to answering these questions:

\begin{itemize}
\item What affects utility more, the fields that are anonymized or the anonymization algorithm?
\item Which fields have a larger impact on the utility of a log?
\item Which anonymization algorithms have a larger impact on the utility of a log?
\end{itemize}

To answer these questions, we evaluated all 152 pairs of fields and
anonymization algorithms. For each pair, the number of alerts
generated by Snort was calculated. The alerts generated for each pair
were compared with the baseline alerts (See
Table~\ref{table:raw-anony1} and Table~\ref{table:raw-anony2}). False
Positives/False negatives were calculated based on the definitions
above, whose detailed results we discuss later.

Although we evaluated all 152 field-anonymization algorithm pairs, we did not include ICMP related fields (such as ICMP\_CHECKSUM, ICMP\_CODE etc) in the results presentend below, since we filtered ICMP packets from the log. There remains a total of 81 field-anonymization pairs.

The unanonymized file produced 81 alerts. The number and types of
alerts produced are summarized in
Table~\ref{table:baseline-alerts}. There are a total of 81 alerts
generated in the baseline file, but only 19 unique types of alerts.

\input{rawAlertData.tex}

\begin{table}[htp]
  \caption{Alerts generated in the baseline unanonymized file. \textbf{AlertID} is the id of the alert; \textbf{Num} is the number of that type of alert generated; \textbf{Desc} is a description of the alert}
  \label{table:baseline-alerts}
  \begin{tabular}[t]{llp{2in}}
    {\textbf{AlertID}} & {\textbf{Num}} & \textbf{Desc} \\
    1 & 1 & (portscan) TCP Portscan \footnote{This alert was generated from generator 122} \\
    323 & 1 & FINGER root query \\
    330 & 1 & FINGER redirection attempt \\
    332 & 1 & FINGER 0 query \\
    356 & 1 &  FTP passwd retrieval attempt \\
    359 & 1 & FTP satan scan \\
    503 & 4 & MISC Source Port 20 to <1024 \\
    1200 & 9 & ATTACK-RESPONSES Invalid UR \\
    1201 & 12 & ATTACK-RESPONSES 403 Forbidden \\
    1288 & 4 &  WEB-FRONTPAGE /\_vti\_bin/ access \\
    1292 & 30 &  ATTACK-RESPONSES directory listing \\
    1418 & 2 & SNMP request tcp \\
    1420 & 2 &  SNMP trap tcp \\
    1421 & 1& SNMP AgentX/tcp request\\
    2467 & 1 & NETBIOS SMB D\$ unicode share access \\
    2470 & 1 & NETBIOS SMB C\$ unicode share access \\
    2473 & 1 & NETBIOS SMB ADMIN\$ unicode share access \\
    3151 & 6 &  FINGER / execution attempt \\
    3441 & 2 & FTP PORT bounce attempt \\
  \end{tabular}
\end{table}


\subsection{Fields or Anonymization Algorithm?}
It is important to understand which causes a greater impact on utility; the field that is being anonymized or the anonymization algorithm that is being applied.

To evaluate the effects of anonymizing a field we calculate the \emph{marginal} of a field. The marginal of a field is the average number of false positive/false negatives over all anonymization algorithms. Similarly the marginal of an anonymization algorithm is the false positive/false negative rate averaged over all fields. The marginal provides a concise summary of the effect of anonymizing a field. 

Figure~\ref{fig:marg-fieldvsfpfn} shows the false positive and false negative marginals of the anonymization algorithms. The full data for this graph is in Table~\ref{tab:marg-fieldFNFP}.

\begin{figure*}[htp]
  \begin{tabular}{cc}
    \includegraphics[width=3in]{./img/marg-fieldvsfp.pdf} & \includegraphics[width=3in]{./img/marg-fieldvsfn.pdf} \\
  \end{tabular}
  \caption{The left hand chart shows the average number of false positive alerts generated for each field. The right hand chart shows the average number of false negative alerts generated for each field.}
  \label{fig:marg-fieldvsfpfn}
\end{figure*}

Figure~\ref{fig:marg-fieldvsfpfn} indicates that the majority of fields generate no false positives or false negatives on average. The fields for which this is true (such as DST\_MAC) did not affect the utility of the log under any anonymization algorithm. We can conclude that anonymizing these fields has no impact on the utility of a log, with respect to the IDS metric. 

The fact that the majority of fields have no impact on utility, even when anonymized in numerous ways, indicates that fields are more important than the anonymization algorithm in determining the utility of an anonymized log. If it was the other way around, we would expect false positives and false negatives to be distributed over all the fields. 

In contrast, if we do the same with anonymization algorithms we see that the majority of anonymization algorithms generate false positives and false negatives, suggesting again that the field has a greater impact on the utility of the log than the anonymization algorithm. Figure~\ref{fig:marg-anonyvsfpfn} shows marginals for anonymization algorithms (averaged over fields). Table~\ref{tab:marg-anonyFNFP} contains the data for the graph. 

We can see in Figure~\ref{fig:marg-anonyvsfpfn} that in terms of false negatives, there are more alerts spread over the set of anonymization algorithms. 

\subsection{Which fields have high impact on utility?}
As Figure~\ref{fig:marg-fieldvsfpfn} and Table~\ref{tab:marg-fieldFNFP} clearly show, the majority of fields do not generate false positives (on average). The fields that do are TCP\_DST\_PORT, TCP\_SRC\_PORT,\\ IPV4\_SRC\_IP, IPV4\_DST\_IP, TS\_SEC, \\ and TCP\_ACK\_NO. 

We can see that several of the fields resulted, in, on average, only 81 alerts. These fields (shown in italics in the table) had 0 error. Judging from these results, we can see that this set of fields did not affect the utility of the log as measured by the IDS metric. 

TCP\_DST\_PORT and TCP\_SRC\_PORT generated the most alerts on
average. Upon inspection of the generated alert files, we can see that
most of the pairs generated only 2 types of alerts. In the case of
BinaryBlackMarker there were 520286 alerts of type 524
generated. Alert 524 is ``BAD-TRAFFIC tcp port 0 traffic''. The other
anonymization algorithms produced the same pattern---the majority of
alerts were of type 524.

The reason for this is due to what we substitute for the port
field. The BinaryBlackMarker, Substitution, NumericTruncation, and
Annihilation algorithms replaced the port field with $0$. This
resulted in the alert for nearly all the packets in the log (See
Table~\ref{tab:anonyparam} for the parameter settings of the
anonymization algorithms). the same problem occurs for the
TCP\_SRC\_PORT field.

The RandomPermutation algorithm replaced the port number with another,
random port number, thus not causing the generation of the BAD-TRAFFIC
alert. It is clear from this, that the false positive rate was greatly
affected by the choice of the substitution port, and another useful
metric may be to count types of new alerts rather than the raw alerts.

Arguably, it is the false negative count that is most important in determining the utility of a log. A low false negative count indicates that no information was lost in the process of anonymization. In terms of false negatives, we find that there are $8$ fields that have an impact on the average false negative rate: TCP\_DST\_PORT,TCP\_FLAGS,TCP\_SRC\_PORT, \\ IPV4\_DST\_IP,IPV4\_SRC\_IP,TCP\_ACK\_NO, \\ TCP\_SEQUENCE,TS\_SEC


\subsection{What anonymization algorithms have high impact on utility?}

Figure~\ref{fig:marg-anonyvsfpfn} summarizes the false positive and
false negative rates with respect to anonymization algorithm. For each
anonymization algorithm, the average false positive/false negative rate
is calculated over all the fields. Table~\ref{tab:marg-anonyFNFP}
contains the data for the graphs.

\begin{figure*}[htp]
  \begin{tabular}{cc}
  \includegraphics[width=3in]{./img/marg-anonyvsfp.pdf} & \includegraphics[width=3in]{./img/marg-anonyvsfn.pdf} \\
  \end{tabular}

  \caption{The left hand chart shows the average number of false positive alerts generated for each anonymization algorithm. The right hand chart shows the average number of false negative alerts generated for each anonymization algorithm.}
  \label{fig:marg-anonyvsfpfn}
\end{figure*}

We can see from these that most anonymization algorithms have an impact on the utility of a log. In contrast, the field data that we saw before showed strong structure in what fields affected utility. When veiwed from the perspective of anonymization algorithms, there is no single anonymization algorithm that stands out. 


It might seem like the substitution algorithm has the largest number
of alerts. However, this is because of the parameter setting used. By
looking at the false negative rate we can see that while substitution
still has a large affect on utility, most of the other algorithms have an
affect as well.


\input{AnonyMarginal.tex} \input{FieldMarginal.tex}
%
%
% \begin{figure}[h]

%   \caption{Anony vs. False Positive Rate}
%   \label{fig:marg-anonyvsfp}
% \end{figure}
% %
% %
% \begin{table}[h]
%   \begin{tabular}[h]{ccccc}
    
%   \end{tabular}
%   \caption{Anony vs. False negative}
%   \label{tab:marg-anonyvsfn}
% \end{table}



% Figure~\ref{fig:marg-fieldvsfn} and Table~\ref{tab:marg-fieldvsfn} summarize the average false negative count over fields. 



% \begin{table}[h]
%   \begin{tabular}[h]{ccccc}
    
%   \end{tabular}
%   \caption{Field vs. False negative}
%   \label{tab:marg-fieldvsfn}
% \end{table}


% In comparison, the same summarization applied to anonymization algorithms is shown in Figure~\ref{fig:marg-anonyvsfn}, Table~\ref{tab:marg-anonyvsfn}, 


% %
% %
% \begin{figure}[h]

%   \caption{Anonymization Algorithm  vs. False Negative}
%   \label{fig:marg-anonyvsfn}
% \end{figure}





% Table~\ref{table:raw-anony1} and Table~\ref{table:raw-anony2} in the Appendix list the results from most of the pairs of anonymization algorithms and fields.  

